LITTLE THINGS in 3D: robust determination of the circular velocity of dwarf irregular galaxies

Dwarf Irregular galaxies (dIrrs) are the smallest stellar systems with extended HI discs. The study of the kinematics of such discs is a powerful tool to estimate the total matter distribution at these very small scales. In this work, we study the HI kinematics of 17 galaxies extracted from the `Local Irregulars That Trace Luminosity Extremes, The HI Nearby Galaxy Survey' (LITTLE THINGS). Our approach differs significantly from previous studies in that we directly fit 3D models (two spatial dimensions plus one spectral dimension) using the software $^\text{3D}$BAROLO, fully exploiting the information in the HI datacubes. For each galaxy we derive the geometric parameters of the HI disc (inclination and position angle), the radial distribution of the surface density, the velocity-dispersion ($\sigma_v$) profile and the rotation curve. The circular velocity (V$_{\text{c}}$), which traces directly the galactic potential, is then obtained by correcting the rotation curve for the asymmetric drift. As an initial application, we show that these dIrrs lie on a baryonic Tully-Fisher relation in excellent agreement with that seen on larger scales. The final products of this work are high-quality, ready-to-use kinematic data ($\textrm{V}_\textrm{c}$ and $\sigma_v$) that we make publicly available. These can be used to perform dynamical studies and improve our understanding of these low-mass galaxies.

==> include/datan/iguess.tex <==
\subsection{Preparing the fit} \label{sec:iguess}

\subsubsection{Assumptions}
Given the large number of parameters (9), it is important to start the fitting algorithm with reasonable initial guesses for each of them. 
First, we decreased the parameter to 8 excluding from the fit the HI surface density.   In practice we normalise the flux locally to the value of the total HI map.
For a full description of this normalisation technique, see the 3DB reference paper \citep{barolo}. Then, we fix the scale height and the systemic velocity as follows:

\begin{itemize}
\item{\textit{HI scale height:}} 3DB includes the possibility to fit the HI scale 
height, this is something exclusive of 3D methods since there are no information about 
the scale height in the integrated 2D velocity field. However, the assumption of a thick
disc is somewhat inconsistent with the 'tilted-ring model' (see Sec. \ref{sec:tring}), 
in the presence of a thick disc  along the line of sight we are accumulating  emission 
form different rings, hence a ring by ring analysis can not incorporate this effect. We 
tested 3DB with different assumptions on the HI scale height and as expected the final 
results are not influenced by these choices.
To be fully consistent, we should set the value of the scale height to 0, however in this case we note that the galactic models made with Barolo have a too sharp cut-off at the border of rings. Therefore, we 
decided to set for all the galaxies a scale height of 100 pc, constant in radius. 
{\bf However, it is interesting to note that the dIrrs have a very shallow potential well and hence, they should have a very thick HI disc especially in the outer regions. For this reason, we are developing a method to take the disc thickness of the gasoues layers into account in the kinematic modelling of HI discs, it will be presented in a future work (Iorio et al., in prep). }
{\bf (More details on the discussion?)}
\newline
\item{\textit{Systemic velocity:}} We fix the systemic velocity to the value calculated as
\begin{equation}
\text{V}_\text{sys}=0.5(\text{V20}_\text{app} + \text{V20}_\text{rec}),
\end{equation}
with \text{V20} the velocity where the flux of the global HI profile reaches the 20\% with respect to the flux peak, while 'app' and 'rec' indicate the approaching and the receding halves of the galaxy. 
\end{itemize}


\subsubsection{Initial guesses}
Furthermore, it is very important to have a good initial estimate also for the geometry of the HI disc, namely for the centre, the inclination and the position angle.
We use three different methods to obtain the initial estimates for these parameters:
\begin{itemize}
\item{\textit{3DB:}} 3DB can automatically estimate the geometrical parameters analysing the 0th moment (HI total map) and the 1th moment (velocity field) of the data cube.
{\bf
The inclination is estimated fitting HI model maps to the observed HI total map, while the position angle is calculated as the orientation of the line that maximises the velocity gradient in the velocity field. Finally, the centre is estimated with the flux-weighted average position of the source. 3DB builds the total map and the velocity field using a source-finding algorithm (DUCHAMP,  \citealt{sourceF}), it separates the source pixels from the noise pixels on the basis of a S/N threshold. As a consequence, the final maps and the estimate of the disc parameters depend on the choice of this threshold. For this reason we repeat this analysis using S/N threshold  ranging from 2.5 to 5.
}
\item{\textit{RingFit:}} We  developed a simple script\footnote{{\tt
https://github.com/iogiul/mhf}} to fit ellipses to the isodensity contours of our total
HI maps (Sec. \ref{sec:mapd}). From the properties of the fitted ellipses we can 
estimate the geometrical parameters of the HI disc at different radii.
\item{\textit{Isophotal fitting of the optical maps:}} Geometrical parameters derived from the V-Band photometry by \cite{HVBand}.
\end{itemize}

\begin{figure} 
 \centering 
 \includegraphics[width=1.\columnwidth]{image/d52iguess.pdf}
 \caption{Initial estimate of the inclination angle for DDO 52 (see Fig. \ref{fig:DDO52}). The left panel shows the results of 3DB,  the right panels shows the results of the fit of the isodensity contours of the HI total map, the red lines shows the inclination of the optical disc. See text for further details.}
\label{fig:d52iguess}
\end{figure}

\begin{figure} 
 \centering 
 \includegraphics[width=1.\columnwidth]{image/d210iguess.pdf}
 \caption{Same as Fig. \ref{fig:d52iguess} but for DDO 210 (see Fig. \ref{fig:DDO210}).}
\label{fig:d210iguess}
\end{figure}
{\bf
Figs. \ref{fig:d52iguess} and \ref{fig:d210iguess} show two examples of the estimate of the inclination angle with the method described above. In the first case (DDO52) the three methods are in great agreement, while in the second case (DDO210) the results are not compatible.
As standard approach we tend to give more weight to the optical information. Therefore,
if the other two estimates are not dramatically different (Fig. \ref{fig:d52iguess}), we fix the galactic centre  to the position of the optical centre and then we use the values of the inclination and of the 
position angle of the stellar disc as the initial guesses in 3DB. When the geometry of the stellar  and the HI disc do not show a clear agreement (Fig. \ref{fig:d210iguess}) or the stellar disc presents peculiar features, as strong bars, we use the other two methods combined with visual inspections to fix the galaxy centre and to 
chose a reasonable initial values for the inclination and the position angle. Further details for each galaxy can be found in Sec. \ref{sec:gls}
Finally, we set the initial values of the circular velocity and the of velocity dispersion respectively to 30 and 8 km/s.
}

